From Complexity to Parsimony: Integrating Latent Class Analysis to Uncover Multimodal Learning Patterns in Collaborative Learning

Multimodal Learning Analytics (MMLA) leverages advanced sensing technologies and artificial intelligence to capture complex learning processes, but integrating diverse data sources into cohesive insights remains challenging. This study introduces a novel methodology for integrating latent class analysis (LCA) within MMLA to map monomodal behavioural indicators into parsimonious multimodal ones. Using a high-fidelity healthcare simulation context, we collected positional, audio, and physiological data, deriving 17 monomodal indicators. LCA identified four distinct latent classes: Collaborative Communication, Embodied Collaboration, Distant Interaction, and Solitary Engagement, each capturing unique monomodal patterns. Epistemic network analysis compared these multimodal indicators with the original monomodal indicators and found that the multimodal approach was more parsimonious while offering higher explanatory power regarding students' task and collaboration performances. The findings highlight the potential of LCA in simplifying the analysis of complex multimodal data while capturing nuanced, cross-modality behaviours, offering actionable insights for educators and enhancing the design of collaborative learning interventions. This study proposes a pathway for advancing MMLA, making it more parsimonious and manageable, and aligning with the principles of learner-centred education.

==> backup.tex <==
% \subsubsection{Motivation}
% 4-codes
% Along the X axis (MR1), a Mann-Whitney test showed that 0 (Mdn=0.439, N=10) was statistically significantly different at the alpha=0.05 level from 1 (Mdn=-0.054, N=46 U=343.000, p=0.014, r=-0.491). Along the Y axis (SVD2), a Mann-Whitney test showed that 0 (Mdn=-0.095, N=10) was not statistically significantly different at the alpha=0.05 level from 1 (Mdn=0.250, N=46 U=212.000, p=0.703, r=0.078).

% 17-codes
% Along the X axis (MR1), a Mann-Whitney test showed that 0 (Mdn=-0.16, N=10) was statistically significantly different at the alpha=0.05 level from 1 (Mdn=0.09, N=46 U=358.50, p=0.006, r=-0.56). Along the Y axis (SVD2), a Mann-Whitney test showed that 0 (Mdn=0.00, N=10) was not statistically significantly different at the alpha=0.05 level from 1 (Mdn=-0.06, N=46 U=235.50, p=0.91, r=-0.02).

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{fig-rq2-motivation.png}
%     \caption{Comparison of epistemic networks generated from 17 monomodal (left) and four multimodal behavioural codes (right) for students with low (red) and high (blue) motivation.}
%     \label{fig-rq2-motivation}
% \end{figure}
